A Review of ERA5 Equatorial Wind Data and Impact on a Space Elevator

This paper uses the ERA5 weather dataset to assess the impact of the wind on an equatorial space elevator. An analytical formulation establishes that the effect of wind on tether inclination and payload capacity can be captured by a single scalar: RMS wind velocity, averaged over air pressure. This formulation clarifies what constitutes excessive wind for a particular elevator and provides a direct link between wind data and elevator design parameters. Analysis of equatorial ERA5 data shows that equatorial wind loading varies strongly with geography with lower values over continents and higher values over oceans, with the majority contribution coming from the lowest 20 km of atmosphere. The data indicate that realistic equatorial winds pose a significant constraint on thin-ribbon elevator designs if align to face the wind. Combining wind and lightning statistics highlights several promising equatorial regions for anchor sites. Finally, the implications of wind loading for elevator design are examined, and several mitigation strategies are discussed to improve survivability and operational payload capacity under realistic wind conditions.

==> Makefile <==
# Add a list of home-made EPS figures here.
EPSFIGURES=


.SUFFIXES: .fig .eps .ps .dvi .bbl .bib .tex .pdf

FIGURES=${wildcard *.fig}
EPSFIGFILES=${FIGURES:.fig=.eps}
TEXFILES=*.tex

all: pdf   

force: rmdone all

#dvi: paper.dvi

#xdvi: paper.dvi
#	xdvi paper.dvi

gv: paper.ps
	gv paper.ps

ps: paper.ps 

pdf: paper.pdf

rmdone:
	rm -f done.flag

done.flag:
	touch done.flag

printerrors:
	@echo "*****************************"; \
	echo Overview of typeset warnings: ; \
        echo "****************************"; \
	grep "Underfull" paper.log; \
	grep "Overfull" paper.log; \
	echo ; \
        echo "***************************"; \
	echo Overview of latex warnings: ; \
        echo "***************************"; \
	grep "LaTeX Warning" paper.log; \
        echo "***************************"; \
	echo ; \
        echo "***************************"; \
	echo Overview of bibtex warnings: ; \
        echo "***************************"; \
        grep ^Warning-- paper.blg; \
	echo "***************************"; \
	echo ; \
        echo "*************************"; \
	echo Overview of latex errors: ; \
        echo "*************************"; \
	grep "^!" paper.log; \
        echo "*************************"; \
	echo

paper.bbl: paper.bib $(TEXFILES) Makefile done.flag
	pdflatex -interaction=batchmode paper.tex || true
#	rm -f $*.dvi
	bibtex -terse $*

paper.pdf: $(TEXFILES) $(EPSFIGFILES) paper.bbl $(EPSFIGURES) Makefile done.flag
	@echo Running latex once.; \
	while ( pdflatex -interaction=nonstopmode paper.tex; grep Rerun paper.log ) ; do \
          echo; \
          echo "*********************************"; \
          echo "*********************************"; \
          echo Reruning to complete compilation.; \
          echo "*********************************"; \
          echo "*********************************"; \
	done; \
        echo "***************************"; \
	echo PDF file generated.; \
        echo "***************************"; \
	echo ; \
	make printerrors 
			
#.ps.pdf: Makefile
#	ps2pdf $< $*.pdf

#.fig.eps: Makefile
#	fig2dev -L pstex $< $*.eps

#.dvi.ps: Makefile
#	dvips -q -P cmz -t letter $< -o $*.ps

#.eps.pdf: Makefile
#	epstopdf $<

clean:
	rm -f *.lof *.lot *.pfg *~ *.aux *.dvi *.blg *.log *.bbl $(EPSFIGFILES) *.bak paper.ps paper.pdf *.toc *.swp done.flag



